Unsupervised 2D-3D lifting of non-rigid objects using local constraints

For non-rigid objects, predicting the 3D shape from 2D keypoint observations is ill-posed due to occlusions, and the need to disentangle changes in viewpoint and changes in shape. This challenge has often been addressed by embedding low-rank constraints into specialized models. These models can be hard to train, as they depend on finding a canonical way of aligning observations, before they can learn detailed geometry. These constraints have limited the reconstruction quality. We show that generic, high capacity models, trained with an unsupervised loss, allow for more accurate predicted shapes. In particular, applying low-rank constraints to localized subsets of the full shape allows the high capacity to be suitably constrained. We reduce the state-of-the-art reconstruction error on the S-Up3D dataset by over 70%.

==> figures/deformingThings4D.tex <==
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=\columnwidth]{figures/DF4D_lioness}
\end{center}
\vspace{-0.2cm}
\caption{\textbf{DeformingThings4D.} 99 frames. Keypoints with less that 30\% visibility are removed and 100 keypoints are selected using furthest-point sampling. Video in the supplementary.
}
\label{fig:df4d}
\vspace{-0.2cm}
\end{figure}



==> figures/teaser.tex <==
% \twocolumn[{%
% \renewcommand\twocolumn[1][]{#1}%
% \maketitle
% \begin{center}
% \centering
% % \captionsetup{type=figure}
% \includegraphics [width=0.93\linewidth]{figures/allrap_teaser.pdf}
% \vspace{-2mm}
% \caption{\textbf{3D Reconstruction for partially-occluded 2D semantic keypoints.} With an orthographic camera model, for visible points ($v=1$) we know the screen coordinates $(x,y)$ and must predict only the depth $z$. For occluded points ($v=0$), we must predict all three $(x,y,z)$-coordinates. At test time, a trained deep network predicts the unknown coordinates. The network is generic, without any kind of low-rank constraints built-in; the geometric intuition is built into the losses during training, see Figure~\ref{fig:splash}. For a perspective camera model, the same process can be applied along the camera rays, rather than directly using the $x$-, $y$- and $z$-axes.}
% \vspace{-2mm}
% \label{fig:teaser}
% \end{center}%
% }]


==> figures/training_curves.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/training_curves.png}
\vspace{-2mm}
\end{center}
\caption{}
\vspace{-2mm}
\label{fig:training_curves}
\end{figure}

==> sec/00_preamble.tex <==
%
% --- inline annotations
%
\def\sup3d{S-Up3D}
\def\nrsfs{ALLRAP}
\usepackage[dvipsnames]{xcolor}
\usepackage{enumerate}%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


